PlaceRAN: Optimal Placement of Virtualized Network Functions in the Next-generation Radio Access Networks

The fifth-generation mobile evolution enables several transformations on Next Generation Radio Access Networks (NG-RAN). The RAN protocol stack is splitting into eight possible disaggregated options combined into three network units, i.e., Central, Distributed, and Radio. Besides that, further advances allow the RAN software to be virtualized on top of general-purpose vendor-neutral hardware, dealing with the concept of virtualized RAN (vRAN). The disaggregated network units initiatives reach full interoperability based on the Open RAN (O-RAN). The combination of NG-RAN and vRAN results in vNG-RAN, enabling the management of disaggregated units and protocols as a set of radio functions. The placement of these functions is challenging since the best decision can be based on multiple constraints, such as the RAN protocol stack split, routing paths of transport networks with restricted bandwidth and latency requirements, different topologies and link capabilities, asymmetric computational resources, etc. This article proposes the first exact model for the placement optimization of radio functions for vNG-RAN planning, named PlaceRAN. The main objective is to minimize the computing resources and maximize the aggregation of radio functions. The PlaceRAN evaluation considered two realistic network topologies. Our results reveal that the PlaceRAN model achieves an optimized high-performance aggregation level, it is flexible for RAN deployment overcoming the network restrictions, and it is up to date with the most advanced vNG-RAN design and development.

==> Tables/Additional.tex <==
\begin{savenotes}
\begin{table}[!h]
    \caption{Additional Setup for Fibre and RAN}
    \label{tab:additional}%
    \centering{ {
        \begin{tabular}{|l|c|c|c|c|c|}
        \hline
        \multicolumn{1}{|c|}{Fibre Inputs} & \multicolumn{5}{c|}{Latency (ms)$^{1}$}  \\ \hline
        
        \rowcolor[HTML]{cdd5e4} WDM Optic & \multicolumn{5}{c|}{0.010625} \\ \hline
      
        WDM Electric  & \multicolumn{5}{c| }{0.0005} \\ \hline
      
       \rowcolor[HTML]{cdd5e4} Fiber ??? & \multicolumn{5}{c|}{0.000005} \\ \hline \hline
      
       \multicolumn{1}{|c|}{RAN Inputs} & Channel & YYY & MIMO & PRB & SPB \\ 
       \multicolumn{1}{|c|}{} & (MHz) &  & (layers) &  & (KHz) \\ \hline
      
      \rowcolor[HTML]{cdd5e4} gNB profile 1 & 40 & 32T32R & 8 & 216 & 15  \\ \hline
      
      gNB profile 2 & 100 & 64T64R & 8 & 132 & 60 \\ \hline 
      
%      \hline
      
%       \multicolumn{2}{|c|}{RU Inputs} & F1 & F3 & Rand1 & Rand2 \\ \hline
       
%       \rowcolor[HTML]{cdd5e4} \multicolumn{2}{|l|}{Number of RUs} & 1 & 3 & 0 to 1 & 0 to 3  \\ \hline
    
       \end{tabular}
    } }
\end{table}
\end{savenotes}


==> Tables/RW-v0.tex <==
% Table generated by Excel2LaTeX from sheet 'RW Table'
\begin{table*}[h!]
  \centering
  \caption{Related Work}
   % \begin{tabular}{p{4em}p{16.855em}cp{6.645em}p{5.145em}cp{6.785em}}
   \resizebox{\textwidth}{!}{
   %\begin{tabular}{p{4em}p{17em}p{7em}p{6em}p{4em}p{4em}p{4em}}
   \begin{tabular}{clccccl}
    \textbf{Works} &
      \textbf{Placement Goal - Formulation Problem} &
      \textbf{Architecture} &
      \textbf{RAN Nodes} &
      \textbf{Split} &
      \textbf{RC Analysis} &
      \textbf{Crosshaul Evaluation} &  \\
    \midrule
    \cite{garcia2018fluidran} &
      CU centralization and evaluation of Latency Edge  &
      C-RAN &
      CU-RU &
      3 &
     \cmark &
      Real fronthaul \\
    \midrule
    \cite{bhamare2018efficient} &
      BBU centralization and minimization of the overall latency &
      C-RAN &
      BBU-RRH &
      - &
      \cmark &
       Synthetic fronthaul  
      \\
    \midrule
    \cite{harutyunyan2020cu} &
      Dynamic CU for minimizing the power consumption in fronthaul &
      NG-RAN &
      CU-DU &
      4 &
      \xmark &
      Synthetic wireless fronthaul \\
    \midrule
    \cite{arouk2017multi} &
      Minimizing the cost of VNF chain on a substrate network &
      C-RAN &
      BBU-RRH &
      1 &
      \cmark &
      Synthetic fronthaul \\
    \midrule
    \cite{mahapatra2017optimal} &
      BBU centroid position &
      C-RAN &
      BBU-RRH &
      1 &
     \xmark &
      Synthetic fronthaul/backhaul     
      \\
    \midrule
    \cite{molner2019optimization} &
      Maximization of DU sources under non-dedicated optical network &
      NG-RAN &
      CU-DU &
      2 &
      \xmark &
      Real fronthaul/backhaul    \\
    \midrule
    \cite{matoussi20205g} &
      Minimizing computational resources and fronthaul bandwidth &
      C-RAN &
      BBU-RRH &
      3 &
      \xmark &
     Synthetic fronthaul     \\
    \midrule
    \cite{song2019clustered} &
      Minimizing Computational costs &
      D-RAN &
      Monolithic &
      1 &
      \cmark &
      -       \\
    \midrule
    \cite{arouk2018cost} &
      Minimizing the network cost &
      C-RAN &
      CU-DU-RU &
      1 &
      \xmark &
     Synthetic crosshaul     \\
    \midrule
    \cite{masoudi2020cost} &
      Minimizing the total cost of ownership by DU pool&
      C-RAN &
      DU-RU &
      4 &
      \xmark &
      Synthetic fronthaul     \\
    \midrule
    \cite{yusupov2018multi} &
     Minimizing the network nodes and latency paths; maximizing the data rate &
      NG-RAN  &
      CU-DU-RU &
      2 &
      \xmark &
     Synthetic crosshaul      \\
      \midrule
    \cite{harutyunyan2018flex5g} &
      Minimize interference and fronthaul utilization to optimize the functional split &
      C-RAN &
      CU-DU &
      4 &
      \xmark &
      Synthetic fronthaul   
      \\
    \midrule
       \cite{murti2020optimization} &
     Minimize the deployment, computation and routing costs & 
      C-RAN &
      CU-DU &
      3 &
      \cmark &
      Real fronthaul   
      \\
    \midrule
    \textbf{PlaceRAN} &
      \textbf{Minimizing computational resources and maximizing vNG-RAN's aggregation} &
      \textbf{NG-RAN} &
      \textbf{CU-DU-RU} &
      \textbf{19} &
      \textbf{\cmark} &
      \textbf{Real Crosshaul}   
      \\
    \bottomrule
    \end{tabular}
   }
  \label{tab:rw}
\end{table*}%

% Table generated by Excel2LaTeX from sheet 'RW Table'
% \begin{table*}[htbp]
%   \centering
%   \caption{Related Works}
%   % \begin{tabular}{p{4em}p{16.855em}cp{6.645em}p{5.145em}cp{6.785em}}
%   \resizebox{\textwidth}{!}{
%   %\begin{tabular}{p{4em}p{17em}p{7em}p{6em}p{4em}p{4em}p{4em}}
%   \begin{tabular}{ccccccc}
%   \textbf{Works} &
%       \textbf{Placement Goal - Formulation Problem} &
%       \textbf{Formulation and/or Algorithm Method} &
%       \textbf{Architecture} &
%       \textbf{RAN Nodes} &
%       \textbf{Split} &
%       \textbf{RC Analysis}
%       \\
%     \midrule
%     \cite{garcia2018fluidran} &
%       CU centralization and evaluation of Latency edge  &
%       Bender´s Method  &
%       C-RAN &
%       CU-RU &
%       3 &
%      \cmark
%       \\
%     \midrule
%     \cite{bhamare2018efficient} &
%       BBU centralization and minimization of the overall latency &
%       ILP and, BnB and SA Heuristic &
%       C-RAN &
%       BBU-RRH &
%       N/S &
%       \cmark
%       \\
%     \midrule
%     \cite{harutyunyan2020cu} &
%       Dynamic CU for minimizing the power consumption in the fronthaul network &
%       ILP and Heurisitc &
%       NG-RAN &
%       CU-DU &
%       4 &
%       \xmark
%       \\
%     \midrule
%     \cite{arouk2017multi} &
%       Minimizing the cost of VNF chain embedding on a substrate network &
%       ILP and Multi-Objective Placement &
%       C-RAN &
%       BBU-RRH &
%       1 &
%       \cmark
%       \\
%     \midrule
%     \cite{mahapatra2017optimal} &
%       BBU centroid position &
%       K-means &
%       C-RAN &
%       BBU-RRH &
%       1 &
%      \xmark
%       \\
%     \midrule
%     \cite{molner2019optimization} &
%       Maximization of DU sources under non-dedicated optical network &
%       Math and Heuristic &
%       NG-RAN &
%       CU-DU &
%       2 &
%       \xmark
%       \\
%     \midrule
%     \cite{matoussi20205g} &
%       Minimizing Computational resources and fronthaul bandwidth &
%       ILP and Heuristic &
%       C-RAN &
%       BBU-RRH &
%       3 &
%       \xmark
%       \\
%     \midrule
%     \cite{song2019clustered} &
%       Minimizing Computational costs &
%       ILP and Graph Partitioning  &
%       D-RAN &
%       Monolithic &
%       1 &
%       \cmark
%       \\
%     \midrule
%     \cite{arouk2018cost} &
%       Minimizing the network cost &
%       MIQCP &
%       C-RAN &
%       CU-DU-RU &
%       1 &
%       \xmark
%       \\
%     \midrule
%     \cite{masoudi2020cost} &
%       Minimizing TCO by DU pool&
%       ILP and GA &
%       C-RAN &
%       DU-RU &
%       4 &
%       \xmark
%       \\
%     \midrule
%     \cite{yusupov2018multi} &
%      Minimizing the network nodes and Latency paths, maximizing the remaining data rate links &
%       MIQCP &
%       NG-RAN  &
%       CU-DU-RU &
%       2 &
%       \xmark
%       \\
%       \midrule
%     \cite{harutyunyan2018flex5g} &
%       Minimize cells interference and fronthaul utilization to optimize the functional split &
%       ILP and Heuristic &
%       C-RAN &
%       CU-DU &
%       4 &
%       \xmark
%       \\
%     \midrule
%       \cite{murti2020optimization} &
%      Minimize the deployment, computation and routing costs. & Benders Method &
%       C-RAN &
%       CU-DU &
%       3 &
%       \cmark
%       \\
%     \midrule
%     OW &
%       Minimizing the CRs nodes and maximizing the aggregation of vNG-RAN functional split & \textcolor{red}{Math Optimization}
%       &
%       NG-RAN &
%       CU-DU-RU &
%       19 &
%       \cmark
%       \\
%     \bottomrule
%     \end{tabular}%
%     }
%   N/S - Not Specified
%   \label{tab:rw}%
%     %\caption{N/S - Not Specified}
% \end{table*}%

%\begin{tabular}{p{4em}p{15em}p{8em}p{4em}p{4em}p{4em}p{4em}}

% \begin{table*}[htbp]
%   \centering
%   \caption{Add caption}
%   % \begin{tabular}{p{4em}p{16.855em}cp{6.645em}p{5.145em}cp{6.785em}}
%   \resizebox{\textwidth}{!}{
%   \begin{tabular}{p{4em}p{17em}p{7em}p{6em}p{4em}p{4em}p{6em}}
%     \multicolumn{1}{c}{\textbf{Work}} &
%       \textbf{Placement Goal} &
%       \multicolumn{1}{p{8.93em}}{\textbf{Algorithm Method}} &
%       \textbf{Architecture} &
%       \textbf{RAN Nodes} &
%       \multicolumn{1}{p{4em}}{\textbf{Split Functional}} &
%       \textbf{Computational Resources}
%       \\
%     \midrule
%     \cite{garcia2018fluidran} &
%       CU centralization and ensure strictly Latency in the edge  &
%       \multicolumn{1}{p{8.93em}}{Bender Decomposition} &
%       C-RAN &
%       CU-RU &
%       3 &
%       CPU
%       \\
%     \midrule
%     \cite{bhamare2018efficient} &
%       BBU centralization and minimizing the overall latency &
%       \multicolumn{1}{p{8.93em}}{BnB and SA Heuristic} &
%       C-RAN &
%       BBU-RRH &
%       \multicolumn{1}{p{4.57em}}{N/A} &
%       CPU and RAM
%       \\
%     \midrule
%     \cite{harutyunyan2020cu} &
%       Dynamic CU for minimizing the power consumption in the fronthaul network &
%       \multicolumn{1}{p{8.93em}}{Heurisitc} &
%       NG-RAN &
%       CU-DU &
%       4 &
%       N/A
%       \\
%     \midrule
%     \cite{arouk2017multi} &
%       Minimizing the cost of VNF chain embedding on a substrate network &
%       \multicolumn{1}{p{8.93em}}{Multi-Objective} &
%       C-RAN &
%       BBU-RRH &
%       1 &
%       CPU and RAM
%       \\
%     \midrule
%     \cite{mahapatra2017optimal} &
%       BBU centroid position &
%       \multicolumn{1}{p{8.93em}}{K-means} &
%       C-RAN &
%       BBU-RRH &
%       1 &
%       N/A
%       \\
%     \midrule
%     \cite{molner2019optimization} &
%       Maximization of DU sources under non-dedicated optical network &
%       \multicolumn{1}{p{8.93em}}{Heurisitc} &
%       NG-RAN &
%       CU-DU &
%       2 &
%       N/A
%       \\
%     \midrule
%     \cite{matoussi20205g} &
%       Minimizing Computaional and link costs &
%       \multicolumn{1}{p{8.93em}}{Particle Swarm Optimization} &
%       C-RAN &
%       BBU-RRH &
%       6 &
%       N/A
%       \\
%     \midrule
%     \cite{song2019clustered} &
%       Minimizing Computaional costs &
%       \multicolumn{1}{p{8.93em}}{Math Model} &
%       C-RAN 3 layers &
%       CU-DU-RU &
%       1 &
%       CPU
%       \\
%     \midrule
%     \cite{arouk2018cost} &
%       Minimizing TCO by DU pool &
%       \multicolumn{1}{p{8.93em}}{Genetic} &
%       C-RAN &
%       DU-RU &
%       1 &
%       N/A
%       \\
%     \midrule
%     \cite{masoudi2020cost} &
%       Minimizing the network nodes and Latency paths, maximizing the remaining data rate links &
%       \multicolumn{1}{p{8.93em}}{Multi-Objective} &
%       C-RAN 3 layers &
%       CU-DU-RU &
%       4 &
%       N/A
%       \\
%     \midrule
%     \cite{yusupov2018multi} &
%       Minimizing number of processing resources &
%       \multicolumn{1}{p{8.93em}}{Math Model} &
%       C-RAN 3 layers &
%       CU-DU-RU &
%       2 &
%       N/A
%       \\
%     \midrule
%     Proposed Work &
%       Minimizing the computanional resources nodes and maximizing the aggregation and centralization of CU and DU nodes &
%       &
%       NG-RAN &
%       CU-DU-RU &
%       19 &
%       CPU and RAM
%       \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:old}%
% \end{table*}%


==> Tables/RW-v1.tex <==
\begin{table*}[!h]
    \caption{Related work.}
    \label{tab:related}
    \centering{ {
        \begin{tabular}{|l|c|l|c|c|c|}
        \hline
        \multicolumn{1}{|c}{Works} & \multicolumn{1}{|c}{RAN} & \multicolumn{1}{|c}{Optimization Goals} & \multicolumn{2}{|c|}{Disaggregated RAN} & \multicolumn{1}{c|}{Transport}  \\ 
        \cline{4-5} 
        \multicolumn{1}{|c}{} & \multicolumn{1}{|c}{Architecture}  & \multicolumn{1}{|c}{} & \multicolumn{1}{|c}{Nodes}  & \multicolumn{1}{|c}{DRCs} & \multicolumn{1}{|c|}{Network} \\ \hline \hline
        
        \rowcolor[HTML]{cdd5e4} \multicolumn{1}{|c|}{\cite{garcia2018fluidran}} & C-RAN & CU centralization and evaluation of Latency Edge & CU-RU & 3 & Fronthaul \\
    
        \multicolumn{1}{|c|}{\cite{fonseca:19}} & \textcolor{red}{NG-RAN} & CU centralization and CU positioning & CU-RU & 5 & Fronthaul/Backhaul \\
        
        \rowcolor[HTML]{cdd5e4}
        \multicolumn{1}{|c|}{\cite{bhamare2018efficient}} & C-RAN & BBU centralization and minimize the overall latency &
        BBU-RRH & - & Fronthaul  \\

        \multicolumn{1}{|c|}{\cite{harutyunyan2020cu}} & NG-RAN & Dynamic CU to minimize the power consumption & CU-DU & 4 & Fronthaul \\
        
        \rowcolor[HTML]{cdd5e4}
        \multicolumn{1}{|c|}{\cite{arouk2017multi}} & C-RAN & Minimize the cost of VNF chain on substrate network & BBU-RRH &
        1 & Fronthaul \\
        
        \multicolumn{1}{|c|}{\cite{mahapatra2017optimal}} &  C-RAN & BBU centroid position & BBU-RRH & 1 & Fronthaul/Backhaul   \\
        
        \rowcolor[HTML]{cdd5e4}
        \multicolumn{1}{|c|}{\cite{molner2019optimization}} & NG-RAN & Maximize DU sources under non-dedicated optical network & CU-DU & 2 & Fronthaul/Backhaul    \\
        
        \multicolumn{1}{|c|}{\cite{matoussi20205g}} &  C-RAN & Minimize CRs and fronthaul bandwidth & BBU-RRH & 3 & Fronthaul \\
        
        \rowcolor[HTML]{cdd5e4}
        \multicolumn{1}{|c|}{\cite{song2019clustered}} & D-RAN & Minimize Computational costs & Monolithic & 1 & -  \\
        
        \multicolumn{1}{|c|}{\cite{arouk2018cost}} & \textcolor{red}{C-RAN} & Minimize the network cost &     CU-DU-RU & 1 & Crosshaul     \\
        
        \rowcolor[HTML]{cdd5e4}
        \multicolumn{1}{|c|}{\cite{masoudi2020cost}} & C-RAN & Minimize the total cost of ownership by DU pool & DU-RU & 4 &  Fronthaul     \\
        
         \multicolumn{1}{|c|}{\cite{yusupov2018multi}} & NG-RAN  & Minimize the nodes and latency; maximize the data rate & CU-DU-RU & 2 & Crosshaul      \\
        
        \rowcolor[HTML]{cdd5e4} 
        \multicolumn{1}{|c|}{\cite{harutyunyan2018flex5g}} & C-RAN & Minimize interference to optimize the utilization and splits & CU-DU & 4 & Fronthaul   \\
        
        \multicolumn{1}{|c|}{\cite{murti2020optimization}, \cite{murti:20}} & \textcolor{red}{NG-RAN} & Minimize the vRAN cost, which involves number and & CU-DU-(RU) & 3 & Crosshaul  \\
        & & locations of CUs and overall routing & & & \\

        \rowcolor[HTML]{3c4563} \multicolumn{1}{|c|}{\color{white} PlaceRAN} & \color{white} NG-RAN  &  \color{white} Minimize CRs and maximize vNG-RAN's aggregation & \color{white} CU-DU-RU & \color{white} 9 & \color{white} Crosshaul \\  \hline

       \end{tabular}
    } }
\end{table*}

==> sections/Introduction_old.tex <==
\section{Introduction}
\label{intro}

\IEEEPARstart {T} {he} current world digital transformation is bringing an explosion of traffic in the mobile network operators \cite{data2019ict}. The fifth-generation of mobile evolution is considered one of the leading enablers of this transformation \cite{data2019ict,radukic2019effects}. A fundamental part of the mobile network, i.e., the running monolithic Radio Access Network (RAN), has several challenges to meet such an evolution. For example, the new standards must design the network's functions closer to the user, aiming to decrease application delay experience \cite{bertenyi2018ng,sectoritu}. Therefore, monolithic RAN must be rethought to meet the desires of digital transformation \cite{ericsson20175g}.


The main standards development organizations specify and guide the RAN supported on the protocol stack disaggregation and the software-based networking. The 3rd Generation Partnership Project (3GPP) \cite{3gpp.23.501}, the International Telecommunication Union Telecommunication (ITU-T) \cite{gstr2018transport}, and European Telecommunications Standards Institute (ETSI) \cite{etsingran} collaborated to specify the next generation RAN (NG-RAN) architecture and the RAN virtualization (vRAN) to meet the new network demands. Furthermore, the industry creates its initiatives for NG-RAN. The most promising are based on open solutions, called Open RAN (O-RAN). The relevant leaderships are OpenRAN, a project group within Telecom Infra Project (TIP), O-RAN Alliance, and Small Cell Forum focused on general-purpose vendor-neutral hardware, software-defined technologies, and interoperability \cite{gavrilovska2020cloud}.

The NG-RAN architecture proposed enables the base station for splitting the protocol stack into the eight options combined into three network elements: (i) Central Unit (CU), (ii) Distributed Unit (DU), and (iii) Radio Unit (RU) \cite{gstr2018transport,marsch20185g}. These split options concern to improve the radio functions and cost efficiency compared with the Distributed RAN (D-RAN) used in the last mobile generations \cite{agrawal2017cloud,marsch20185g}. Distinct from the predecessor architecture, Cloud RAN (C-RAN) centralizes the baseband and operates with a single split in the fronthaul transport network for communication between the BaseBand Unit (BBU) and the Remote Radio Head (RRH) \cite{al20185g}. Although NG-RAN seeks to overcome the old architecture, it has the prerogative to support C-RAN, D-RAN, and DU-RU integration scenarios. Moreover, the O-RAN industry initiative follows this splitting model, including the "open" word for network nodes, creating the O-CU, O-DU, and O-RU nomenclature \cite{o-ran1}.

The network software process in NG-RAN is guided by the virtualization of nodes and radio functions by the Network Function Virtualization (NFV) concept \cite{badulescu2019etsi,bernardos2019network}. For example, the NG-RAN architecture functional split combined with vRAN provides flexibility for mobile access networks. The most concrete model proposed is the O-RAN Alliance, which explores six virtualized and physical radio functions scenarios centralized on cloud computing and distributed on edge computing  \cite{o-ran1}. This flexibility allows mobile network operators to place the radio functions in a way that takes into account available network resources and user demand (e.g., ultra-low latency and high-bandwidth applications). The placement of radio functions in a fine-grained network management approach is considered vital for fifth-generation networks to achieve the expected leadership of digital transformation. However, the development of the virtualized NG-RAN architecture (vNG-RAN) is an unprecedented challenging problem since crosshaul transport networks (backhaul, midhaul, and fronthaul) have restricted bandwidth and latency requirements, different topologies and link capabilities, asymmetric computing resources (CR), and unbalanced user demand \cite{gstr2018transport,sehier2019transport}. 


%In addition to evaluating cost and performance strategies.

vNG-RAN is up-to-date in fifth-generation research, although no decision-making method for specification designing of the placement of virtualized radio network functions is defined. The placement problem is defined on the optimal optimization (or the closest to the optimal) based on the best joint decision between the split of the RAN protocol stack, the routing paths of the crosshaul network, and the CRs strategies the CU, DU, and RU nodes \cite{laghrissi2018survey}. Therefore, the ideal placement leads to analysis related to the bandwidth and latency requirements for each split option between CU-DU and DU-RU. Moreover, each split option results in a computing cost (processing, memory, and storage) to be evaluated. According to the network's scalability, the placement needs to be aware of the load occupation, even for routing paths and computing resources allocation. In this case, a combinatorial analysis makes constructing an NP-hard type challenging optimization algorithm due to the high volume of possibilities to design the vNG-RAN \cite{masdari2016overview,laghrissi2018survey}. %\textcolor{blue}{(Esse parágrafo precisa refetir o Related Work, i.e., introduzindo o gap existente na literatura. Precisa citar explicitamente alguns artigos que fazem algo marginal, mas não o que esse trabalho se propõe.)}

In the literature, several works lead to the placement optimization of radio functions. However, these works mostly address specific strategies to perform the placement, the C-RAN architecture and applied approximate or heuristic algorithms to achieve a close to an optimal solution. In this sense, the main strategies developed highlight BBU/CU's position for C-RAN architecture (low functional splits options) \cite{garcia2018fluidran,bhamare2018efficient,mahapatra2017optimal}, financial costs \cite{arouk2018cost,masoudi2020cost}, efficiency under crosshaul constraints (mainly, the fronthaul network) \cite{yusupov2018multi,murti2020optimization,harutyunyan2020cu}, and computing resources \cite{song2019clustered,arouk2017multi}. Therefore, to the best of our knowledge, there is no work in the literature (i) focusing on the disaggregated vNG-RAN with high functional split options and protocol stack analysis, (ii) aligning O-RAN industry strategies, (iii) optimizing computing resources and crosshaul paths, and (iv) bringing exact approaches.

% This article proposes the PlaceRAN optimal algorithm for the placement optimization of radio functions for network planning and evaluation of vNG-RAN.

%PlaceRAN algorithm is composed of three stages with independent Objective Functions (OF), and for each stage, the crosshaul and CR constraints are evaluating. The three OFs are sequentially complementary, according to:

\textbf{Contributions}. In this article, we introduce PlaceRAN, the problem formulation for the optimal placement of vNG-RAN functions. The problem is formulated as the best trade-off between maximizing the aggregation level of virtualized NG-RAN functions and minimizing the amount of computing resources necessary for running these functions. PlaceRAN innovates by considering in the formulation all RAN elements (RU, DU, and CU), the paths between these elements (fronthaul, midhaul, and backhaul), and also all functional splits according to the standards. Our contributions can be summarized as follows:

\begin{itemize}
    
    \item \textbf{New problem formulation} -- in some aspects, PlaceRAN is the most general problem formulation in the context of vNG-RAN, and it was designed with a comprehensive set of real-world NG-RANs considerations in mind.

    \item \textbf{New approach} -- to properly formulate PlaceRAN, we introduced some concepts, such as Disaggregated RAN Combination (DRC) and multi-stage problem formulation, turning the problem formulation simple despite its generality.

    \item \textbf{Efficient exact solution} -- despite the problem complexity, we were able to solve PlaceRAN using a conventional solver (i.e., IBM CPLEX) for real-world RAN instances.
    
    \item \textbf{Evaluation and new insights} -- our evaluation employed examples of present and future RANs. We show how PlaceRAN can contribute with the virtualization of present RANs, but it also ready to deal with the optimal placement of forthcoming vNG-RANs. 
    
     \item \textbf{Relevant results} -- the results show no standard configuration for vNG-RAN and the PlaceRAN model presents the necessary flexibility to overcoming the network constraints achieving the aggregation levels above 80\% up to two centralized nodes near of core.
     
     %support to leverage the required flexibility, despite all , we observe aggregation levels above 80 \% centralized in nodes a hop from the network core.
    
    
%    \hl{As examples of new insights, we observed ...}.
    
\end{itemize}

%\textbf{Contributions}. This article proposes an exact model for the placement optimization of radio functions for network planning and evaluation of vNG-RAN, named PlaceRAN. The main objective is to minimize the computing resources and maximize the aggregation of radio functions of vNG-RAN (achieve the maximum of protocol stack aggregation and, consequently, concentrating several RUs in a single DU and several DUs in a single CU). Two other specific objectives are unfolded. For the first, the PlaceRAN model guarantees the minimization of the number of Disaggregated RAN Combination (DRC), which maps the possibilities of combinations of functional splits elaborated and contributed by the authors. The second is the flexibility to prioritize DRCs according to industry and standard developer organizations' strategies to deploy vNG-RAN. For example, prioritize O-RAN Alliance splits options. 

%For all objectives, the crosshaul and CR constraints are evaluating through mathematical optimization models.

%The PlaceRAN approach is composed of three stages. In each stage the crosshaul and CR constraints are evaluating through mathematical optimization models. \textcolor{blue}{Destacar as principais contribuições do artigo:}



%this article proposes the PlaceRAN optimization algorithm for the placement of the radio functions in the vNG-RAN architecture. The proposal's main goal is to \textcolor{blue}{maximize the CU and DU elements} hierarchy proposed by the NG-RAN architecture. PlaceRAN is composed of three stages. The first stage defines the number the computing resources used to place the CU and DU elements for the optimal solution. After, the second stage determines the optimal placement based on the first stage's input. \textcolor{blue}{In finally, the third stage...} In this sense, the algorithm aims to make the RAN split's best choice decision and allocate c resources to overcome the crosshaul network's constraints.  

% For example, the disaggregation benefits result for large-scale networks in spectral efficiency,  better handover, overhead reduction, etc.

%The proposal's main goal is to \textcolor{blue}{maximize the CU and DU elements} hierarchy proposed by the NG-RAN architecture since, for large-scale networks, the disaggregation benefits resulting in the radio spectrum's efficiency, dual connectivity, handover, and overhead reduce. 

%In this context, the RAN nodes are virtualized in common-off-the-shelf (COTS) hardware in a multitasking computing infrastructure (cloud and edge computing) overlayed under the crosshaul network. 

%To evaluate the PlaceRAN model and obtain significant insights that contribute to the fifth-generation development, we analyzed PlaceRAN in two real crosshaul network datasets that present the projects topologies 5G-crosshaul (T1) \cite{5G-crosshaul} and PASSION (T2) \cite{passion}. In which T1 is designed to meet current demands, and T2 envisions evolving requirements. Regarding the analysis of CRs, our article also brings reality with computing parameters and metrics available and evaluated in the industry to characterize their impact on vNG-RAN. Finally, the optimization coverage also supports C-RAN, D-RAN, and DU-RU architectures to extract the best crosshaul and RAN.

%To evaluate the PlaceRAN approach and obtain significant insights that contribute to the fifth-generation development, we analyzed PlaceRAN in real crosshaul network datasets of 5G-crosshaul \cite{5G-crosshaul} and  PASSION \cite{passion} projects. These datasets present different topologies and a great diversity of distances, which significantly impact the latency parameter. Regarding the analysis of CRs, our article also brings reality with computing parameters and metrics available and evaluated in the industry to characterize their impact on vNG-RAN. Finally, the optimization coverage also supports C-RAN, D-RAN, and DU-RU architectures to extract the best crosshaul and RAN.

%\textcolor{blue}{(Precisamos trazer aqui algum resultado impactante)}. In this sense, 
%The PlaceRAN extracts the best decision for choosing the disaggregation of vNG-RAN, allocating CRs, and overcoming the crosshaul network's constraints. Therefore, PlaceRAN is fully qualified to be applied in other real datasets with different characteristics since it supports legacy and future networks. Our contributions can be summarized as follows:

% \begin{itemize}
    
%     \item PlaceRAN Math Approach - An exact mathematical model for vNG-RAN placement for network planning.

%     \item PlaceRAN Placement Optimization - To the best of our knowledge, this is the first work that develops the vNG-RAN architecture and a relevant number of DRCs.

%     \item PlaceRAN Targets - Minimize computing resources, leverage radio functions with maximum aggregation, reduce the number of DRCs (homogeneous network), and make the implementation strategy flexible. All of this overcoming crosshaul constraints.

    
% \end{itemize}
    % \item The OF's first stage defines the number of CRs in line with the RAN protocols' aggregations.
    % \item The second stage assesses OF based on minimizing the number of Disaggregated RAN Combination (DRC). DRCs are the authors' evaluation and consequent contribution to the possible combinations of the RAN breakdown.
    % \item The third stage defines OF based on the DRCs weights of industry and standard developer organization strategy to deploy the vNG-RAN. For example, prioritize O-RAN Alliance splits options. 
    
%    \item For each stage, the crosshaul and CR constraints are evaluating. ---> movi para o parágrafo anterior.

% Finally, based on the PlaceRAN evaluation, we show a significant improvement in high-scale networks and alignment with the operational networks. For example, the PlaceRAN performance results show up to 80\% of RAN VNFs aggregation centralized in the CU nodes.


\textbf{Article organization.} Section \ref{sec:concepts} introduces the vNG-RAN background. The PlaceRAN system model and problem statement are described in Section \ref{sec:model}. Section \ref{evaluation} presents the PlaceRAN evaluation methodology and results. The related work is discussed in Section \ref{rw}, and finally, Section \ref{conc} presents the final remarks.

% the datasets evaluate, and introduces the system model. Section \ref{design} provides the problem’s formulation, while Section \ref{metho} presents the solution method. Section \ref{evaluation} presents a full evaluation of the PlaceRAN orchestrator. The literature review is discussed in Section \ref{rw} and the final remarks in Section \ref{conc}.

%Context\\
%Problem\\
%Motivation\\
%Literature summary\\
%Contributions
